Reversible Random Walks on Dynamic Graphs

Recently, random walks on dynamic graphs have been studied because of their adaptivity to the time-varying structure of real-world networks. In general, there is a tremendous gap between static and dynamic graph settings for the lazy simple random walk: Although $O(n^3)$ cover time was shown for any static graphs of $n$ vertices, there is an edge-changing dynamic graph with an exponential hitting time. On the other hand, previous works indicate that the random walk on a dynamic graph with a time-homogeneous stationary distribution behaves almost identically to that on a static graph. In this paper, we strengthen this insight by obtaining general and improved bounds. Specifically, we consider a random walk according to a sequence $(P_t)_{t\geq 1}$ of irreducible and reversible transition matrices such that all $P_t$ have the same stationary distribution. We bound the mixing, hitting, and cover times in terms of the hitting and relaxation times of the random walk according to the worst fixed $P_t$. Moreover, we obtain the first bounds of the hitting and cover times of multiple random walks and the coalescing time on dynamic graphs. These bounds can be seen as an extension of the well-known bounds of random walks on static graphs. Our results generalize the previous upper bounds for specific random walks on dynamic graphs, e.g., lazy simple random walks and $d_{\max}$-lazy walks, and give improved and tight upper bounds in various cases. As an interesting consequence of our generalization, we obtain tight bounds for the lazy Metropolis walk [Nonaka, Ono, Sadakane, and Yamashita, TCS10] on any dynamic graph: $O(n^2)$ mixing time, $O(n^2)$ hitting time, and $O(n^2\log n)$ cover time. Additionally, our coalescing time bound implies the consensus time bound of the pull voting on a dynamic graph.

==> Metropolis/sections/cover_time.tex <==
\section{Cover time}
\label{sec:cover_time}

%\color{red} (proof based on Matthew's argument?)
%Consider a walk $(X_t)_{t\geq 0}$ according to $\Pseq=(P_t)_{t\geq 1}$.
%For fixed vertices $u$ and $v$,
%let $\tau_{\mathrm{hit}}(u\to v)$ be first time that
%the walk visit $v$ starting from $u$.
%Then, from the Markov inequality, for $T\defeq \mathrm{e}\thit$,
%we have $\Pr[\tau_{\mathrm{hit}}(u\to v) \geq T]\leq 1/\mathrm{e}$.
%Moreover, for any $\ell$, $\Pr[\tau_{\mathrm{hit}}(u\to v)\geq \ell T] \leq (1/\mathrm{e})^\ell$.
%To see this, divide the walk of length $\ell T$
%into $\ell$ consecutive walks each of length $T$.
%Each of these walk visits $v$ with probability at least $1-1/\mathrm{e}$ regardless of the initial position.
%Hence, by the Markov property, we obtain the claim.


%\begin{lemma}[$k$-Hitting Time]
%Consider $k$ independent walks $(X_t)_{t\geq 0}$
%for $X_t=(X_t(1),\dots,X_t(k))\in V^k$ where each walk $(X_t(i))_{t\geq 0}$ is according to $\Pseq=(P_t)_{t\geq 0}$
%such that $\Pseq$ has the time-homegeneous stationary distribution $\pi$.
%Suppose that the walks start from $x=(x_1,\dots,x_k)\in V^k$ (i.e., $X_0(i)=x_i$ for all $i\in[k]$).
%For $y\in V$,
%let $\tau_{\mathrm{hit}}^{(k)}(x,y)=\inf\{t\geq 0:X_t(i)=y\text{ for some $i\in[k]$}\}$
%and $\thit^{(k)}=\max_{x,y}\tau_{\mathrm{hit}}^{(k)}(x,y)$.
%Then, $\thit^{(k)}=O(\thit / k)$.
%$\thit^{(k)}=O(\thit / k)$.
%\end{lemma}


%Similarly,
%if we consider $k$ independent walks each of length  $\ell T'$ with $T'=\mathrm{e}\thit^{(k)}$,
%the probability that these walks does not
%visit $v$ is at most $(1/\mathrm{e})^{\ell}$.
%By the union bound over $v\in V$,
%we obtain
%$\Pr_{x}[\tau_{\mathrm{cov}}^{(k)} \geq \ell T'] \leq n\mathrm{e}^{-\ell}$.
%In other words,
%$\Pr_x[\tau^{(k)}_{\mathrm{cov}}/T' -\log n\geq \ell] \leq \mathrm{e}^{-\ell}$
%and thus $\E_x[\tau^{(k)}_{\mathrm{cov}}/T' -\log n]=O(1)$.
%Therefore, we have
%\begin{align*}
%    \tcov^{(k)}&=\max_x\E[\tau^{(k)}_{\mathrm{cov}}]  \\
%    &\leq (T'+O(1))\log n \\
%    &\leq O(\log n+\thit\log n/k).
%\end{align*}
%\color{black}

We prove \cref{thm:main}\ref{lab:rev_cov}.
Consider
$k$ independent random walks $(X_t(1))_{t\geq 0},\ldots,(X_t(k))_{t\geq 0}$ according to $\Pseq$.
Let $(X_t)_{t\geq 0}$ be a random variable defined as $X_t=(X_t(1),\ldots,X_t(k))\in V^k$.
Let $\tauhit^{(k)}(\Pseq,w)$ (for $w\in V$) and $\taucov^{(k)}(\Pseq)$ be the
random variables denoting hitting and cover times of the $k$ random walks, respectively.
That is,
\begin{align*}
    \tauhit^{(k)}(\Pseq,w)&=\inf\left\{t\geq 0:\bigcup_{i\in[k],0\leq s\leq t} \{X_s(i)\} \ni w \right\},\\
    \taucov^{(k)}(\Pseq) &= \inf\left\{t\geq 0:\bigcup_{i\in [k],0\leq s\leq t}\{X_s(i)\}=V\right\}.
\end{align*}
We sometimes abbreviate $\Pseq$ and write $\tauhit^{(k)}(w)$ and$\taucov^{(k)}$
    if $\Pseq$ is clear from the context.

\begin{lemma}
\label{lem:covleq}
Let $\Pseq=(P_t)_{t\geq 1}$ be a sequence of transition matrices.
Suppose that $\Pseq$ is reversible with respect to a probability vector $\pi\in (0,1]^V$ and
contains an irreducible and lazy subsequence $\Pseq'=(P_{t(i)})_{i\geq 1}$ having an interval at most $C$.
Then, for any $k$, $T\geq 2Ct_m^{(\pi)}(\Pseq')+C\left\lceil \frac{8\hitmax(\Pseq')\log(50n)}{k}\right \rceil$, and $x\in V^k$,
$
\Pr\left[\bigvee_{w\in V}\bigwedge_{i\in [k]}\bigwedge_{t=0}^{T}\{X_t(i)\neq w\}\middle| X_0=x\right]
\leq \frac{99}{100}
$ holds.
\end{lemma}
\begin{proof}
%Let $\mathcal{X}=(X_t(1),\ldots,X_t(k))_{t=0}^\infty$ denote $k$ independent random walks according to $\Pseq$, respectively.
Write $t_m=2Ct_m^{(\pi)}(\Pseq')$ for convenience.
From \cref{thm:uniform_mixing}, there is a transition matrix $q\in [0,1]^{V\times V}$ such that
\begin{align*}
%\Pr[X_{s+2t_m}(i)=u|X_s(i)=x_i]
(P_{1}P_{2}\cdots P_{t_m})(x,u)
=\frac{1}{4}\pi(u)+\frac{3}{4}q(x,u)
%\label{eq:covsep}
\end{align*}
holds for any $x,u\in V$.
%
Write $\mathcal{E}$ denote the event that $\bigvee_{w\in V}\bigwedge_{i\in [k]}\bigwedge_{t=0}^{T}\{X_t(i)\neq w\}$ for convenience.
Now, we apply \cref{lem:probprod} to $\mathcal{E}$ with the following settings:
For $S\subseteq [k]$ and $i\in [k]$, define the probability distribution $\mu_{S,i}\in [0,1]^V$ by $\mu_{S,i}\defeq \mathbbm{1}_{i\in S}\pi+\mathbbm{1}_{i\notin S}q(x_i,\cdotp)$.
Let $I_1, I_2, \ldots, I_k$ be $k$ independent binary random variables such that $\Pr[I_i=1]=1/4$ holds for any $i\in [k]$ and let $I=\{i\in [k]: I_i=1\}$.
Let $\mathcal{U}=\{S\subseteq [k]: |S|\geq k/8\}$.
%
From \cref{lem:probprod},
%
\begin{align}
&\Pr\left[\mathcal{E}\middle| X_0=x\right]\nonumber \\
&\leq \Pr[I\notin \mathcal{U}]+\max_{S\in \mathcal{U}}\sum_{u=(u_1,\ldots,u_k)\in V^k}\Pr\left[\mathcal{E}\middle|X_{t_m}=u,X_0=x\right]\prod_{i\in [k]}\mu_{S,i}(u_i)
\label{eq:main_cov}
\end{align}
holds for any $x\in V^k$.
From the Chernoff inequality (\cref{lem:Chernoff}), it is easy to see that
\begin{align}
\Pr[I\notin \mathcal{U}]
&=\Pr\left[\sum_{i=1}^kI_i\leq k/8\right]
\leq \exp\left(-\frac{k}{32}\right).
\label{eq:boundexp_cov}
\end{align}
Note that $\E\left[\sum_{i=1}^kI_i\right]=k/4$.
For the second term of \cref{eq:main_cov}, from the union bound and the Markov property, we have
\begin{align*}
\Pr\left[\mathcal{E}\middle|X_{t_m}=u,X_0=x\right]
&\leq \sum_{w\in V}\Pr\left[\bigwedge_{i\in [k]}\bigwedge_{t=t_m}^{T}\{X_t(i)\neq w\}\middle|X_{t_m}=u\right]\nonumber \\
&\leq \sum_{w\in V}\prod_{i\in [k]}\Pr\left[\bigwedge_{t=t_m}^{T}\{X_t(i)\neq w\}\middle|X_{t_m}(i)=u_i\right]\nonumber \\
&=\sum_{w\in V}\prod_{i\in [k]}\left(Q_{w,[t_m+1,T]}\mathbbm{1}\right)(u_i).
%\label{eq:decomp_cov}
\end{align*}
%Write $f(u_i)=\Pr\left[\bigwedge_{t=s+t_m}^{s+T}\{X_t(i)\neq w\}\middle|X_{s+t_m}(i)=u_i\right]=\left(Q_{w,[s+t_m+1,s+T]}\mathbbm{1}\right)(u_i)$ for convenience.
Note that the equality follows from \cref{eq:thitmeetmatrix}.
Hence, 
\begin{align}
&\sum_{u=(u_1,\ldots,u_k)\in V^k}\Pr\left[\mathcal{E}\middle|X_{t_m}=u,X_0=x\right]\prod_{i\in [k]}\mu_{S,i}(u_i)\nonumber \\
&\leq \sum_{w\in V}\sum_{u_1\in V,\ldots, u_k\in V}\prod_{i\in [k]}\mu_{S,i}(u_i)\prod_{i\in [k]}\left(Q_{w,[t_m+1,T]}\mathbbm{1}\right)(u_i)\nonumber \\
&=\sum_{w\in V}\prod_{i\in [k]}\sum_{u_i\in V}\mu_{S,i}(u_i)\left(Q_{w,[t_m+1,T]}\mathbbm{1}\right)(u_i)\nonumber \\
&\leq \sum_{w\in V}\prod_{i\in S}\sum_{u_i\in V}\pi(u_i)\left(Q_{w,[t_m+1,T]}\mathbbm{1}\right)(u_i)
\label{eq:distributionmatrixcov}
\end{align}
holds for any $S\in \mathcal{U}$.
By assumption, $(P_t)_{t=t_m+1}^{T}$ contains an irreducible subsequence with length of $\lfloor (T-t_m)/C \rfloor =\left\lceil \frac{8\hitmax(\Pseq')\log(50n)}{k}\right \rceil\geq \frac{8\hitmax(\Pseq')\log(50n)}{k}$.
Applying \cref{lem:mainhit}, 
\begin{align}
&\sum_{w\in V}\prod_{i\in S}\sum_{u_i\in V}\pi(u_i)\left(Q_{w,[t_m+1,T]}\mathbbm{1}\right)(u_i)\nonumber \\
&\leq \sum_{w\in V}\prod_{i\in S}\exp\left(-\frac{8\log(50n)}{k}\right) %\nonumber \\
=\sum_{w\in V}\exp\left(-|S|\frac{8\log(50n)}{k}\right) %\nonumber\\
%\leq n\exp\left(-\log(50n)\right)
\leq \frac{1}{50}.
\label{eq:bound_cov1}
\end{align}
holds for any $S\in \mathcal{U}$.
Combining \cref{eq:main_cov,eq:boundexp_cov,eq:distributionmatrixcov,eq:bound_cov1}, 
$
\Pr\left[\mathcal{E}\middle| X_0=x\right]
\leq \exp\left(-\frac{1}{32}\right)+\frac{1}{50}\leq \frac{99}{100}
$.
\end{proof}
%

\begin{proof}[Proof of \cref{thm:main}\ref{lab:rev_cov}]
For $\mathcal{X}=(X_t)_{t\geq 0}=((X_t(1),\ldots,X_t(k)))_{t\geq 1}$, 
let $\mathcal{E}(\mathcal{X},[a,b])$ be the event of $\bigvee_{w\in V}\bigwedge_{i\in [k]}\bigwedge_{t=a}^{b}\{X_t(i)\neq w\}$.
Then, for any $x\in V^k$, $s\geq 0$, we have $\Pr[\mathcal{E}(\mathcal{X},[s,s+T])|X_s=x]\leq 99/100$.
Here, $T\defeq 2Ct_m^{(\pi)}(\Pseq')+C\left\lceil \frac{8\hitmax(\Pseq')\log(50n)}{k}\right \rceil$.
To see this, consider the following arguments.
Let $\Pseq^*=(P^*_t)_{t\geq 1}$ be a sequence of transition matrices, where $P^*_t\defeq P_{s+t}$ for all $t\geq 1$.
Let $(X_t^*(1))_{t\geq 0},\ldots,(X_t^*(k))_{t\geq 0}$ be $k$ independent random walks, where each walk is according to $\Pseq^*$.
Write $X_t^*=(X_t^*(1),\ldots,X_t^*(k))$ for each $t\geq 0$.
Then, since $\Pr[X_{s+t}(i)=v|X_s(i)=u]=\Pr[X_{t}^*(i)=v|X_0^*(i)=u]$ holds for any  $u,v\in V$ and $i\in [k]$, we obtain $\Pr[\mathcal{E}(\mathcal{X},[s,s+T])|X_s=x]=\Pr[\mathcal{E}(\mathcal{X}^*,[0,T])|X_0^*=x]\leq 99/100$. Here, we use \cref{lem:covleq}.

Write $\mathcal{E}_{a,b}=\mathcal{E}(\mathcal{X},[a,b])$ and $\mathcal{E}[\ell]=\bigwedge_{i=1}^\ell\mathcal{E}_{(i-1)T,iT}$ for convenience.
Then, $\Pr[\taucov(\Pseq)>\ell T|X_0=x]\leq \Pr\left[\mathcal{E}[\ell]\middle| X_0=x\right]$ and
%
\begin{align*}
%&\Pr[\taucov(\Pseq)>\ell T|X_0=x]\\
&\Pr\left[\mathcal{E}[\ell]\middle| X_0=x\right]\\
&=\sum_{x'\in V^k}\Pr\left[\mathcal{E}_{(\ell-1)T,\ell T}, \mathcal{E}[\ell-1], X_{(\ell-1)T}=x'\middle| X_0=x\right]\\
&=\sum_{x'\in V^k}\Pr\left[\mathcal{E}_{(\ell-1)T,\ell T}\middle| \mathcal{E}[\ell-1], X_{(\ell-1)T}=x', X_0=x\right] \Pr\left[ \mathcal{E}[\ell-1], X_{(\ell-1)T}=x'\middle| X_0=x\right]\\
&=\sum_{x'\in V^k}\Pr\left[\mathcal{E}_{(\ell-1)T,\ell T}\middle| X_{(\ell-1)T}=x'\right]  \Pr\left[ \mathcal{E}[\ell-1], X_{(\ell-1)T}=x'\middle| X_0=x\right]\\
&\leq 99/100\Pr\left[ \mathcal{E}[\ell-1]\middle| X_0=x\right]
\leq \cdots \leq \left(99/100\right)^\ell.
\end{align*}
Hence, we have
\begin{align*}
\E[\taucov(P)|X_0=x]
&=\sum_{\ell=0}^\infty \sum_{t=0}^{T-1}\Pr[\taucov(P)>\ell T + t|X_0=x]
\leq T\sum_{\ell=0}^\infty \left(99/100\right)^\ell
\leq 100T.
\end{align*}
\end{proof}



%


==> Metropolis/sections/hitting_time.tex <==

\section{Hitting and meeting time lemmas}
\label{sec:hitting_time}
We introduce \cref{lem:mainhit,lem:mainmeet}, which enable us to bound the hitting, cover and coalescing times for the random walk $(X_t)_{t\geq 0}$ according to a sequence of transition matrices $\Pseq$.
For $w\in V$, define $D_w\in \{0,1\}^{V\times V}$ by $D_w(u,v)\defeq \mathbbm{1}_{u=v}\mathbbm{1}_{u\neq w}$ for each $u,v\in V$. 
%\begin{align}
%D_w(u,v)\defeq 
%\begin{cases}
%1&(\textrm{if $u=v$ and $u\neq w$}) \\
%0 &(\textrm{otherwise})
%\end{cases},
%\end{align}
%i.e., an $n \times n$ identity matrix with $D_w(w,w)=0$.
For $\Pseq=(P_t)_{t\geq 1}$ and a sequence of vertices $\mathcal{W}=(w_t)_{t\geq 0}$, 
let $Q_{\mathcal{W},t}\defeq D_{w_{t-1}}P_t D_{w_t}$ and $Q_{\mathcal{W},[a,b]}\defeq Q_{\mathcal{W},a}Q_{\mathcal{W},a+1}\cdots Q_{\mathcal{W},b}$ for $1\leq a\leq b$.
Then, 
\begin{align}
\Pr\left[\bigwedge_{t=a-1}^b\{X_t\neq w_t\}\middle| X_{a-1}=\cdot \right] 
= D_{w_{a-1}}P_aD_{w_{a}}P_{a+1}D_{w_{a+1}} \cdots P_{b}D_{w_{b}} \mathbbm{1}
=Q_{\mathcal{W},[a,b]}\mathbbm{1}
\label{eq:thitmeetmatrix}
\end{align}
holds for any $1\leq a\leq b$.
If $\mathcal{W}=(w_t)_{t\geq 0}$ satisfies $w_t=w\in V$ for all $t$, 
write $Q_{w,t}=D_wPD_w$ and $Q_{w,[a,b]}=Q_{w,a}Q_{w,a+1}\cdots Q_{w,b}$ for abbreviation.
%
\subsection{Hitting time}
We introduce the following lemma, which is a special case of the Meeting Time Lemma (\cref{lem:MTL}) in the dynamic setting.
The result plays a key role to bound the hitting time (\cref{thm:main}\ref{lab:rev_hit}) and the cover time (\cref{sec:cover_time}).
Here, we do not assume aperiodicity or laziness.
%\begin{restatable}{lemma}{mainhit}
\begin{lemma}
\label{lem:mainhit}
For any $T\geq 0$, $w\in V$ and sequence of transition matrices $\Pseq=(P_t)_{t=1}^T$ that is irreducible and reversible with respect to a probability vector $\pi\in (0,1]^V$, 
%Let $(P_t)_{t=a}^b$ be a sequence of transition matrices on $V$.
%Suppose that $(P_t)_{t=a}^b$ is reversible with respect to a probability vector $\pi\in (0,1]^V$ and contains an irreducible subsequence $\Pseq'=(P_{t(i)})_{i=1}^L$.
%Let $H_*=\max_{i\in [L]}\thit(P_{t(i)})$.
%Then, for any $w\in V$,
\begin{align*}
%sum_{v\in V}\pi(v)\left(Q_{w,[a,b]}\mathbbm{1}\right)(v) 
%\Pr\left[\tau_w(\Pseq)>T\right]
%\leq 
\left\|Q_{w,[1,T]}\mathbbm{1}\right\|_{2,\pi}
\leq \exp\left(-\frac{T}{\thitmax(\Pseq)}\right).
\end{align*}
\end{lemma}
\paragraph{Remark.}
\Cref{lem:mainhit} implies that
\begin{align*}
    \sum_{v\in V}\pi(v)\Pr\left[\tau_w(\Pseq)>T|X_0=v\right]\leq \left\|Q_{w,[1,T]}\mathbbm{1}\right\|_{2,\pi}\leq \exp\left(-\frac{T}{\thitmax(\Pseq)}\right)
\end{align*}
holds. The first inequality follows from \cref{eq:thitmeetmatrix} and the Cauchy-Schwarz inequality.
%It is not difficult to see that, for any $t>0$, \cref{lem:mainhit} implies
%\begin{align*}
%    \left\|Q_{w,[t,t+T]}\mathbbm{1}\right\|_{2,\pi}\leq \exp\left(-\frac{T}{\thitmax(\Pseq)}\right).
%\end{align*}
\begin{proof}[Proof of \cref{lem:mainhit}]
%The first inequality is trivial from the Cauchy-Schwarz inequality.
%For the second inequality, 
Applying \cref{lem:MatrixEigen} repeatedly yields
\begin{align*}
\left\|Q_{w,[1,T]}\mathbbm{1}\right\|_{2,\pi}
&=\left\|Q_{w,1}Q_{w,[2,T]}\mathbbm{1}\right\|_{2,\pi}
\leq \rho\left(Q_{w,1}\right)\left\|Q_{w,[2,b]}\mathbbm{1}\right\|_{2,\pi}
\leq \cdots \leq \prod_{t=1}^T\rho\left(Q_{w,t}\right).
\end{align*}
%From \cref{lem:hiteigen}, $\rho(D_{w,t(i)})\leq 1-\frac{1}{\thit(P_{t(i)})}$ holds for any $i\in [L]$.
Hence, from \cref{lem:hiteigen},
\begin{align*}
\prod_{t=1}^T\rho\left(Q_{w,t}\right)
%\leq \prod_{i\in [L]}\rho\left(D_{w,t(i)}\right)
\leq \prod_{t=1}^T\left(1-\frac{1}{\thit(P_{t})}\right) 
\leq \exp\left(-\sum_{t=1}^T\frac{1}{\thit(P_{t})}\right)
\leq \exp\left(-\frac{T}{\thitmax(\Pseq)}\right)
\end{align*}
holds and we obtain the claim.
%Note that $\rho\left(Q_{w,t}\right)\leq 1$ holds for any $t$.
\end{proof}
%


%\begin{lemma}
%\label{lem:hit_const}
%Let $(X_t)_{t\geq 0}$ be the random walk according to $\Pseq=(P_t)_{t\geq 1}$, that is reversible with respect to a probability vector $\pi\in (0,1]^V$.
%Then, $\Pr\left[ \tau_w(\Pseq)>T \middle| X_0=x\right]\leq 1/2$ holds for any $x,w\in V$
%if $(P_t)_{t=1}^{T}$ contains an irreducible and apperiodic subsequence $\Pseq'=(P'_i)_{i=1}^L=(P_{t(i)})_{i=1}^{L}$ with $L\geq \tgmix^{(2,\pi)}(\Pseq')+\hitmax(\Pseq')$.
%\end{lemma}
%
%\begin{proof}
%From \cref{eq:thitmeetmatrix}, we have $\Pr\left[ \tau_w(\Pseq)>T \middle| X_0=x\right]=\Pr\left[ \bigwedge_{t=0}^T\{X_t\neq w\} \middle| X_0=x\right]=\left(Q_{w,[1,T]}\mathbbm{1}\right)(x)$ for any $x\in V$.
%Write $t_m=\tgmix^{(2,\pi)}(\Pseq')$.
%Applying \cref{lem:mainhit} yields
%\begin{align*}
%\left(Q_{w,[1,T]}\mathbbm{1}\right)(x)
%&=\sum_{v\in V}Q_{w,[1,t(t_m)]}(x,v)\left(Q_{w,[t(t_m)+1,T]}\mathbbm{1}\right)(v)\\
%&\leq \sum_{v\in V}P_{w,[1,t(t_m)]}(x,v)\left(Q_{w,[t(t_m)+1,T]}\mathbbm{1}\right)(v)\\
%&\leq \sqrt{\sum_{v\in V}\frac{P_{w,[1,t(t_m)]}(x,v)^2}{\pi(v)}\sum_{v'\in V}\pi(v')\left(Q_{w,[t(t_m)+1,T]}\mathbbm{1}\right)(v')^2 }\\
%&=\sqrt{1+d^{(2,\pi)}(P_{[1,t(t_m)]}(x,\cdotp))^2} \left\|Q_{w,[t(t_m)+1,T]}\mathbbm{1}\right\|_{2,\pi}\\
%&\leq \sqrt{1+1/4}\exp\left(-\frac{\hitmax(\Pseq')}{\hitmax(\Pseq')}\right)\leq \frac{1}{2}.
%\end{align*}
%We use \cref{eq:l2variance} in the second equality.
%Note that $(P_t)_{t=1}^{t(t_m)}$ contains $(P_{t(i)})_{i=1}^{t_m}$ and $(P_t)_{t=t(t_m)+1}^{T}$ contains $(P_{t(i)})_{i=t_m+1}^{L}$.
%\end{proof}
%


%
%\begin{proof}[Proof of \cref{thm:mainhit}]
%From \cref{eq:thitmeetmatrix}, it holds for any $x,w\in V$ that
%\begin{align*}
%\Pr\left[\tau_w(\Pseq)>T\middle| X_0=x\right]=\Pr\left[\bigwedge_{t=0}^T\{X_t\neq w\}\middle| X_0=x\right]= \left(Q_{w,[1,T]}\mathbbm{1}\right)(x).
%\end{align*}
%Write $t_m=\tmix^{(2,\pi)}(\Pseq)$. 
%For any $T\geq t_m$, 
%Then, 
%\begin{align*}
%\Pr\left[\tau_w(\Pseq)>T\middle| X_0=x\right]
%\left(Q_{w,[1,T]}\mathbbm{1}\right)(x)
%&=\sum_{v\in V}Q_{w,[1,t_m]}(x,v)\left(Q_{w,[t_m+1,T]}\mathbbm{1}\right)(v) \\
%&\leq \sum_{v\in V}P_{[1,t_m]}(x,v)\left(Q_{w,[t_m+1,T]}\mathbbm{1}\right)(v) \\
%&\leq \sqrt{\sum_{v\in V}\frac{P_{[1,t_m]}(x,v)^2}{\pi(v)}\sum_{v'\in V}\pi(v')\left(Q_{w,[t_m+1,T]}\mathbbm{1}\right)(v')^2} \\
%&=\sqrt{1+d^{(2,\pi)}(P_{[1,t_m]}(x,\cdotp))^2}\left\| Q_{w,[t_m+1,T]}\mathbbm{1}\right\|_{2,\pi}\\
%&\leq \sqrt{1+1/4}\exp\left(-\frac{\lfloor (T-t_m)/C \rfloor}{\hitmax(\Pseq')}\right)
%    \leq 2\exp\left(-\frac{T-t_m}{C\hitmax(\Pseq')}\right)
%\label{eq:Qwabhit1}
%\end{align*}
%holds  from \cref{lem:mainhit}.
%We use \cref{eq:l2variance} in the second equality.
%Note that $(P_{t})_{t=t_m+1}^T$ contains an irreducible subsequence with length at least $\lfloor (T-t_m)/C \rfloor$.
%\begin{align*}
%    \Pr\left[\tau_w(\Pseq)>T\middle| X_0=x\right]
%    \leq \sqrt{1+1/4}\exp\left(-\frac{\lfloor (T-t_m)/C \rfloor}{\hitmax(\Pseq')}\right)
%    \leq 2\exp\left(-\frac{T-t_m}{C\hitmax(\Pseq')}\right).
%\end{align*}
%Hence, for any $x\in V$, 
%\begin{align*}
%\E\left[\tau_w(\Pseq)\middle| X_0=x\right]
%&=\sum_{T=0}^\infty\Pr\left[\tau_w(\Pseq)>T\middle| X_0=x\right]\\
%&\leq t_m+1+\sum_{T=t_m+1}^\infty 2\exp\left(-\frac{T-t_m}{C\hitmax(\Pseq')}\right) \\
%&=t_m+1+2\sum_{T=1}^\infty \exp\left(-\frac{T}{C\hitmax(\Pseq')}\right)
%&\leq t_m+1+2C\hitmax(\Pseq').
%\end{align*}
%holds for any $x\in V$ and $T\geq t_m$.
%The last inequality follows since
%$
%\sum_{t=1}^\infty \exp(-tc)
%\leq \frac{\exp(-c)}{1-\exp(-c)}
%=\frac{1}{\exp(c)-1}
%\leq \frac{1}{c}
%\label{eq:useful_inverse_expo}
%$ 
%holds. % for any $c>0$.

%\end{proof}

%\color{red}
%\begin{theorem}
%\label{thm:mainkhit}
%Let $\Pseq=(P_t)_{t\geq 1}$ be a sequence of transition matrices on $V$.
%Suppose that $\Pseq$ is reversible with respect to a positive probability vector $\pi\in (0,1]^V$ and
%contains an irreducible subsequence $\mathcal{P'}=(P_{t(i)})_{i\geq 1}$ having an interval at most $C$.
%Let $H_*=\max_{i}\thit(P_{t(i)})$.
%Then, 
%\begin{align*}
%\thit^{(k)}(\Pseq)
%\leq \tmix^{(2,\pi)}(\Pseq)+\frac{\log 2}{C\hitmax(\Pseq')}+2+\frac{2C\hitmax(\Pseq')}{k}.
%\end{align*}
%\end{theorem}
%\begin{proof}
%Consider
%$k$ independent walks $(X_t)_t$ with $X_t=(X_t(1),\dots,X_t(k))\in V^k$.
%Let $t_m'\defeq t_m+ \lceil \log 2/(C\hitmax(\Pseq'))\rceil$.
%Then, because of the independence of the walks, for any $w\in V$ and $x=(x_1,\dots,x_k)\in V^k$,
%we have
%\begin{align*}
%\E\left[\tau^{(k)}_w(\Pseq)\middle| X_0=x\right]
%&=\sum_{T=0}^\infty\prod_{i=1}^k\Pr\left[\tau_w(\Pseq)>T\middle| X_0(i)=x_i\right]\\
%&\leq t'_m+1+\sum_{T=t'_m+1}^\infty \exp\left(k\log 2-\frac{k(T-t_m)}{C\hitmax(\Pseq')}\right) \\
%&\leq t'_m+1+\sum_{T=t'_m+1}^\infty \exp\left(-\frac{k(T-t'_m)}{C\hitmax(\Pseq')}\right) \\
%&\leq 
%\end{align*}
%\end{proof}
%\color{black}

%%%
\subsection{Meeting time lemma for lazy chains}
%
Consider two independent random walks $(X_t(1))_{t\geq 0}$ and $(X_t(2))_{t\geq 0}$, where each walk is 
according to $\Pseq=(P_t)_{t\geq 1}$. 
%For each $t$, write $X_t=(X_t(1),X_t(2))\in V^2$ for convenience.
The meeting time is defined by $\tmeet(\Pseq)\defeq \max_{x,y\in V}\E[\taumeet(\Pseq)|X_0(1)=x,X_0(2)=y]$, where $\taumeet(\Pseq)\defeq \min\{t\geq 0: X_t(1)=X_t(2)\}$. 
Now, we have the following: 
For any $0\leq s< a\leq b$ and $x,y\in V$, there is a sequence of vertices $\mathcal{W}^*=\{w^*_t\}_{t\geq 0}$ such that
\begin{align}
\Pr\left[\bigwedge_{t=a-1}^b\{X_t(1)\neq X_t(2)\}\middle| \begin{array}{c}X_{a-1}(1)=x,\\ X_{s}(2)=y\end{array}\right]&\leq \left(Q_{\mathcal{W}^*,[a,b]}\mathbbm{1}\right)(x)
\label{eq:tmeetmatrix}
\end{align}
holds.
It is because
\begin{align*}
&\Pr\left[\bigwedge_{t=a-1}^b\{X_t(1)\neq X_t(2)\}\middle| \begin{array}{c}X_{a-1}(1)=x,\\ X_{s}(2)=y\end{array}\right] \nonumber \\
&=\sum_{\substack{(w_t)_{t=a-1}^b\\\in V^{b-a+2}}}\Pr\left[\bigwedge_{t=a-1}^b\{X_t(1)\neq w_t\}\middle|X_{a-1}(1)=x\right]\Pr\left[\bigwedge_{t=a-1}^b\{X_t(2)= w_t\}\middle|X_{s}(2)=y\right] \nonumber \\
&\leq \max_{\substack{(w_t)_{t=a-1}^b\in V^{b-a+2}}}\Pr\left[\bigwedge_{t=a-1}^b\{X_t(1)\neq w_t\}\middle|X_{a-1}(1)=x\right] 
=  \left(Q_{\mathcal{W}^*,[a,b]}\mathbbm{1}\right)(x)
\end{align*}
holds for some $\mathcal{W}^*=\{w^*_t\}_{t\geq 0}$.
%
The following lemma plays a key role to bound \cref{eq:tmeetmatrix} and the coalescing time (\cref{sec:coalescing_time}).
%The proof is in \cref{sec:omitted_proof_section_4} due to the page limitation.
%\begin{restatable}{lemma}{mainmeet}
\begin{lemma}
\label{lem:mainmeet}
For any $T\geq 0$, sequence of vertices $\mathcal{W}=(w_t)_{t=0}^{T}$ and sequence of transition matrices $\Pseq=(P_t)_{t=1}^T$ that is irreducible, lazy and  reversible with respect to a  probability vector $\pi\in (0,1]^V$,
%Let $(P_t)_{t=a}^b$ be a sequence of transition matrices on $V$. 
%Suppose that $(P_t)_{t=a}^b$ is reversible with respect to a positive probability vector $\pi\in (0,1]^V$ and 
%contains an irreducible and lazy subsequence $\Pseq'=(P_{t(i)})_{i=1}^L$.
%Let $H_*=\max_{i\in [L]}\thit(P_{t(i)})$.
%Then, for any sequence of vertices $\mathcal{W}=(w_t)_{t={a-1}}^{b}$, 
\begin{align*}
%\sum_{v\in V}\pi(v)\left(Q_{\mathcal{W},[a,b]}\mathbbm{1}\right)(v) \leq 
\left\|Q_{\mathcal{W},[1,T]}\mathbbm{1}\right\|_{2,\pi}
\leq \exp\left(-\frac{T}{\thitmax(\Pseq)}\right).
\end{align*}
\end{lemma}
\begin{proof}
%The first inequality is trivial from the Cauchy-Schwarz inequality.
%In the following, we show the second inequality.
For any $1\leq t\leq T$, applying \cref{lem:normmeet,lem:hiteigen} yields
\begin{align}
\left\|Q_{\mathcal{W},[t,T]}\mathbbm{1} \right\|_{2,\pi}^2
&=\left\|Q_{\mathcal{W},t}Q_{\mathcal{W},[t+1,T]}\mathbbm{1} \right\|_{2,\pi}^2 
=\left\|D_{w_{t-1}}P_{t}D_{w_{t}}Q_{\mathcal{W},[t+1,T]}\mathbbm{1} \right\|_{2,\pi}^2 \nonumber \\
&\leq \rho\left(D_{w_{t-1}}P_{t}D_{w_{t-1}}\right)\rho\left(D_{w_{t}}P_{t}D_{w_{t}}\right) \left\|Q_{\mathcal{W},[t+1,T]}\mathbbm{1} \right\|_{2,\pi}^2 \nonumber \\
&\leq \left(1-\frac{1}{\thit(P_{t})}\right)^2\left\|Q_{\mathcal{W},[t+1,T]}\mathbbm{1} \right\|_{2,\pi}^2.
\label{eq:lazymeetb}
\end{align}
%Since 
%\begin{align}
%\left\|Q_{\mathcal{W},[t,b]}\mathbbm{1} \right\|_{2,\pi}
%&=\left\|Q_{\mathcal{W},t}Q_{\mathcal{W},[t+1,b]}\mathbbm{1} \right\|_{2,\pi} \nonumber \\
%&\leq \rho\left(Q_{\mathcal{W},t}\right)\left\|Q_{\mathcal{W},[t+1,b]}\mathbbm{1} \right\|_{2,\pi} \nonumber \\
%&\leq \left\|Q_{\mathcal{W},[t+1,b]}\mathbbm{1} \right\|_{2,\pi}
%\label{eq:notlazymeetb}
%\end{align}
%holds for any $t\in [a,b]$, 
Applying \cref{eq:lazymeetb} repeatedly, we have% yields
\begin{align*}
\left\|Q_{\mathcal{W},[1,T]}\mathbbm{1} \right\|_{2,\pi}^2
&\leq \prod_{t=1}^T\left(1-\frac{1}{\thit(P_{t})}\right)^2
\leq \exp\left(-\sum_{t=1}^T\frac{2}{\thit(P_{t})}\right)
\leq \exp\left(-\frac{2T}{\thitmax(\Pseq)}\right).
%\label{eq:recmeet}
\end{align*}
%This implies the claim.
%Note that $\thit(P_{t(i)})\leq \hitmax(\Pseq')$ for all $i\in [L]$ by definition.
%Note that $\rho(Q_{\mathcal{W},t})\leq 1$ holds for any $t$.
%In the second inequality, we use \cref{lem:normmeet}.
\end{proof}
%




%%


==> Metropolis/sections/meeting_time_lemma.tex <==
\section{Meeting time lemma}

\subsection{Meeting time lemma for lazy chains}
\begin{lemma}[Meeting Time Lemma on dynamic graphs; Reminder of \cref{lem:MTL}] \label{lem:MTL_formal}
Let $(X_t)_{t\geq 0}$ be a
    random walk according to $\mathcal{P}=(P_t)_{t\geq 1}$
    that is irreducible, lazy, and
    reversible with respect to a
    distribution $\pi\in(0,1]^V$.
Suppose that $X_0$ is sampled
    from $\pi$.
Then,
    for any sequence $w_1,\dots,w_T$ of vertices,
\begin{align*}
    \Pr\left[\bigwedge_{t=0}^T\{X_t\neq w_t\}\right] \leq \exp\left(-\frac{T}{\thitmax(\mathcal{P})}\right).
\end{align*}
\end{lemma}
\begin{proof}
For $w\in V$, define a matrix $D_w\in \{0,1\}^{V\times V}$ by $D_w(u,v)=1$ if $u=v\neq w$ and $D_w(u,v)=0$ otherwise.
For $\mathcal{P}=(P_t)_{t\geq 1}$ and a sequence of vertices $\mathcal{W}=(w_t)_{t\geq 0}$, 
let $Q_{\mathcal{W},t}\defeq D_{w_{t-1}}P_t D_{w_t}$ and $Q_{\mathcal{W},[a,b]}\defeq Q_{\mathcal{W},a}Q_{\mathcal{W},a+1}\cdots Q_{\mathcal{W},b}$ for $1\leq a\leq b$.
Then, 
\begin{align*}
\Pr\left[\bigwedge_{t=a-1}^b\{X_t\neq w_t\}\middle| X_{a-1}=\cdot \right] 
= D_{w_{a-1}}P_aD_{w_{a}}P_{a+1}D_{w_{a+1}} \cdots P_{b}D_{w_{b}} \mathbbm{1}
=Q_{\mathcal{W},[a,b]}\mathbbm{1}
%\label{eq:thitmeetmatrix}
\end{align*}
holds for any $1\leq a\leq b$.

We claim
\begin{align}
%\sum_{v\in V}\pi(v)\left(Q_{\mathcal{W},[a,b]}\mathbbm{1}\right)(v) \leq 
\left\|Q_{\mathcal{W},[1,T]}\mathbbm{1}\right\|_{2,\pi}
\leq \exp\left(-\frac{T}{\thitmax(\mathcal{P})}\right). \label{eq:MTL_norm_bound}
\end{align}
For any $1\leq t\leq T$, applying \cref{lem:normmeet,lem:hiteigen} yields
\begin{align*}
\left\|Q_{\mathcal{W},[t,T]}\mathbbm{1} \right\|_{2,\pi}^2
&=\left\|Q_{\mathcal{W},t}Q_{\mathcal{W},[t+1,T]}\mathbbm{1} \right\|_{2,\pi}^2 
=\left\|D_{w_{t-1}}P_{t}D_{w_{t}}Q_{\mathcal{W},[t+1,T]}\mathbbm{1} \right\|_{2,\pi}^2 \nonumber \\
&\leq \rho\left(D_{w_{t-1}}P_{t}D_{w_{t-1}}\right)\rho\left(D_{w_{t}}P_{t}D_{w_{t}}\right) \left\|Q_{\mathcal{W},[t+1,T]}\mathbbm{1} \right\|_{2,\pi}^2 \nonumber \\
&\leq \left(1-\frac{1}{\thit(P_{t})}\right)^2\left\|Q_{\mathcal{W},[t+1,T]}\mathbbm{1} \right\|_{2,\pi}^2.
\end{align*}
Applying this inequality repeatedly, we have
\begin{align*}
\left\|Q_{\mathcal{W},[1,T]}\mathbbm{1} \right\|_{2,\pi}^2
&\leq \prod_{t=1}^T\left(1-\frac{1}{\thit(P_{t})}\right)^2
\leq \exp\left(-\sum_{t=1}^T\frac{2}{\thit(P_{t})}\right)
\leq \exp\left(-\frac{2T}{\thitmax(\mathcal{P})}\right).
%\label{eq:recmeet}
\end{align*}

From \cref{eq:MTL_norm_bound}, we have
\begin{align*}
\Pr\left[\bigwedge_{t=0}^T\{X_t\neq w_t\}\right]
&= \sum_{v\in V}\sqrt{\pi(v)}\left(\sqrt{\pi(v)}Q_{\mathcal{W},[1,T]}\mathbbm{1}(v)\right) \\
&\leq \sqrt{\sum_{v\in V}\pi(v)}\cdot \sqrt{\sum_{v\in V} \pi(v)Q_{\mathcal{W},[1,T]}\mathbbm{1}(v)^2} \\
&\leq \|Q_{\mathcal{W},[1,T]}\mathbbm{1}(v)\|_{2,\pi} \\
&\leq \exp\left(-\frac{T}{\thitmax(\mathcal{P})}\right).
\end{align*}
Here, we used the Cauchy--Schwartz inequality.

\end{proof}
%


\subsection{Meeting time lemma for nonlazy chains}

The laziness condition of \cref{lem:MTL_formal}
    is essential
    if we consider an
    aperiodic Markov chain
    (e.g., simple random walks
    on bipartite graphs).
However, we can remove this condition
    in the assumption that $w_t$ are the same vertices.
    
\begin{lemma} \label{lem:MTL_nonlazy}
Let $(X_t)_{t\geq 0}$ be a
    random walk according to $\mathcal{P}=(P_t)_{t\geq 1}$
    that is irreducible and
    reversible with respect to a
    distribution $\pi\in(0,1]^V$.
Suppose that $X_0$ is sampled
    from $\pi$.
Then,
    for any $w\in V$,
\begin{align*}
    \Pr\left[\bigwedge_{t=1}^T\{X_t\neq w\}\right] \leq \exp\left(-\frac{T}{\thitmax(\mathcal{P})}\right).
\end{align*}
\end{lemma}
\begin{proof}
It suffices to prove that
\begin{align*}
\left\|Q_{w,[1,T]}\mathbbm{1}\right\|_{2,\pi}
\leq \exp\left(-\frac{T}{\thitmax(\mathcal{P})}\right).
\end{align*}
If $\mathcal{W}=(w_t)_{t\geq 0}$ satisfies $w_t=w\in V$ for all $t$, 
write $Q_{w,t}=D_wPD_w$ and $Q_{w,[a,b]}=Q_{w,a}Q_{w,a+1}\cdots Q_{w,b}$ for abbreviation.
%The first inequality is trivial from the Cauchy-Schwarz inequality.
%For the second inequality, 
Applying \cref{lem:MatrixEigen} repeatedly yields
\begin{align*}
\left\|Q_{w,[1,T]}\mathbbm{1}\right\|_{2,\pi}
&=\left\|Q_{w,1}Q_{w,[2,T]}\mathbbm{1}\right\|_{2,\pi}
\leq \rho\left(Q_{w,1}\right)\left\|Q_{w,[2,b]}\mathbbm{1}\right\|_{2,\pi}
\leq \cdots \leq \prod_{t=1}^T\rho\left(Q_{w,t}\right).
\end{align*}
%From \cref{lem:hiteigen}, $\rho(D_{w,t(i)})\leq 1-\frac{1}{\thit(P_{t(i)})}$ holds for any $i\in [L]$.
Hence, from \cref{lem:hiteigen},
\begin{align*}
\prod_{t=1}^T\rho\left(Q_{w,t}\right)
%\leq \prod_{i\in [L]}\rho\left(D_{w,t(i)}\right)
\leq \prod_{t=1}^T\left(1-\frac{1}{\thit(P_{t})}\right) 
\leq \exp\left(-\sum_{t=1}^T\frac{1}{\thit(P_{t})}\right)
\leq \exp\left(-\frac{T}{\thitmax(\mathcal{P})}\right)
\end{align*}
holds and we obtain the claim.
%Note that $\rho\left(Q_{w,t}\right)\leq 1$ holds for any $t$.
\end{proof}



%%

